Approximately Counting and Sampling Hamiltonian Motifs in Sublinear Time

Counting small subgraphs, referred to as motifs, in large graphs is a fundamental task in graph analysis, extensively studied across various contexts and computational models. In the sublinear-time regime, the relaxed problem of approximate counting has been explored within two prominent query frameworks: the standard model, which permits degree, neighbor, and pair queries, and the strictly more powerful augmented model, which additionally allows for uniform edge sampling. Currently, in the standard model, (optimal) results have been established only for approximately counting edges, stars, and cliques, all of which have a radius of one. This contrasts sharply with the state of affairs in the augmented model, where algorithmic results (some of which are optimal) are known for any input motif, leading to a disparity which we term the ``scope gap" between the two models. In this work, we make significant progress in bridging this gap. Our approach draws inspiration from recent advancements in the augmented model and utilizes a framework centered on counting by uniform sampling, thus allowing us to establish new results in the standard model and simplify on previous results. In particular, our first, and main, contribution is a new algorithm in the standard model for approximately counting any Hamiltonian motif in sublinear time. Our second contribution is a variant of our algorithm that enables nearly uniform sampling of these motifs, a capability previously limited in the standard model to edges and cliques. Our third contribution is to introduce even simpler algorithms for stars and cliques by exploiting their radius-one property. As a result, we simplify all previously known algorithms in the standard model for stars (Gonen, Ron, Shavitt (SODA 2010)), triangles (Eden, Levi, Ron Seshadhri (FOCS 2015)) and cliques (Eden, Ron, Seshadri (STOC 2018)).

==> marco-copy.tex <==

\newcommand{\comment}[1]{\hfill  \textcolor{gray}
{/* \emph{\small #1} */} }

\newcommand{\bitset}{\{0,1\}}
\newcommand{\eps}{\epsilon}
\newcommand{\light}{\textsf{light}}
\newcommand{\heavy}{\textsf{heavy}}
\renewcommand{\ll}{\textsf{$\ell-\ell$}}
\newcommand{\hh}{\textsf{$h-h$}}
\newcommand{\lh}{\textsf{$\ell-h$}}
\newcommand{\davg}{d_{avg}}
\newcommand{\poly}{\mathrm{poly}}

\newcommand{\Ex}{\mathbb{E}}
\newcommand{\Var}{\mathbb{V}}
\newcommand{\eqdef}{\stackrel{\rm def}{=}}

\renewcommand{\th}{\textsuperscript{th}}

%\newcommand{\cy}{c}
%\newcommand{\F}{\textsf{F}}
\newcommand{\F}{\textsf{F}}
\newcommand{\K}{\textsf{K}}
\newcommand{\C}{\textsf{C}}
\newcommand{\Cy}{\textsf{c}}
\newcommand{\Cyk}{{\textsf{C}}_{k}}
\newcommand{\cyk}{n_{\C}}
\newcommand{\ocyk}{\overline{n}_k}
\newcommand{\cl}{n^{\leq \ogamma}_{\F}}
\newcommand{\cmh}{n^{> \ogamma}_{\F}}
\newcommand{\Bl}{B^{\leq \ogamma}}
\newcommand{\Bmh}{B^{> \ogamma}}
\newcommand{\Bm}{B^{(\ogamma,\sqrt{\om}]}}
\newcommand{\Bh}{B^{> \sqrt{\om}}}
\newcommand{\clk}{n^{\leq \ogamma}_k}
\newcommand{\cmhk}{n^{> \ogamma}_k}
\newcommand{\plk}{p^{\leq \ogamma}_k}
\newcommand{\pmhk}{p^{> \ogamma}_k}
%\newcommand{\Cy}{\widetilde{C}}
\newcommand{\f}{\textsf{f}}
\newcommand{\Q}{G_{\Cy}}
\newcommand{\onC}{\overline{n}_{\C}}





\newcommand{\calA}{{\mathcal{A}}}
\newcommand{\calU}{{\mathcal{U}}}
\newcommand{\mA}{{\mathcal{A}}}
\newcommand{\calB}{{\mathcal{B}}}
\newcommand{\calC}{{\mathcal{C}}}
\newcommand{\nc}{C}
\newcommand{\wC}{{\widetilde{C}}}
\newcommand{\calD}{{\mathcal{D}}}
\newcommand{\calG}{{\mathcal{G}}}
\newcommand{\mG}{{\mathcal{G}}}
\newcommand{\calL}{{\mathcal{L}}}
\newcommand{\calP}{{\mathcal{P}}}
\newcommand{\calT}{{\mathcal{T}}}
\newcommand{\oeps}{\overline{\eps}}
%\newcommand{\oeps}{\eps'}



%\newcommand{\trn}{{\widetilde{n}}}
% \newcommand{\trn}{{n_\Delta}}
\newcommand{\trn}{{n'}}
%\newcommand{\trG}{{\widetilde{G}}}
\newcommand{\trG}{{G'}}
%\newcommand{\trm}{{\widetilde{m}}}
\newcommand{\trm}{{m'}}
%\newcommand{\trA}{{\widetilde{\calA}}}
\newcommand{\trA}{{\calA'}}
%\newcommand{\treps}{{\widetilde{\eps}}}
\newcommand{\treps}{{\eps'}}
%\newcommand{\trR}{{\widetilde{R}}}
\newcommand{\trR}{{R'}}
%\newcommand{\tre}{{\widetilde{e}}}
\newcommand{\tre}{e'}


\newcommand{\ogamma}{\overline{\gamma}}
\newcommand{\hgamma}{\widehat{\gamma}}
\newcommand{\od}{\overline{d}_{avg}}

\newcommand{\oD}{\overleftarrow{D}}

%\newcommand{\om}{\overline{m}}
\newcommand{\om}{\overline{m}}
\newcommand{\hm}{\widehat{m}}
\newcommand{\kappaF}{\kappa_{\F}}
%\newcommand{\hc}{\hat{C}}
%\newcommand{\countF}{C}
\newcommand{\vecV}{\overrightarrow{V}}
\newcommand{\hnF}{\widehat{n}_{\F}}
\newcommand{\countF}{n_{\F}}
\newcommand{\cF}{n_{\F}}
\newcommand{\hF}{h_{\F}}
\renewcommand{\S}{\textsf{S}}
\newcommand{\countS}{n_{\S}}
%\newcommand{\countK}{n_{\tiny K_k}}
\newcommand{\countK}{n_{\tiny \K}}
\newcommand{\odelta}{\overline{\delta}}
%\renewcommand{\c}{C}
\newcommand{\onF}{\overline{n}_{\F}}
\newcommand{\onK}{\overline{n}_{K}}
\newcommand{\EX}{\mathbb{E}}
%\newcommand{\ham}{\rm ham}
\newcommand{\ham}{\mathcal{H}}
\newcommand{\countC}{n_{\C}}
%\newcommand{\onC}{\overline{n}_{\C}}


\newcommand{\Sup}{\textrm{Sup}}


\newcommand\numberthis{\addtocounter{equation}{1}\tag{\theequation}}

%\newenvironment{proof}{\smallskip\noindent{\bf Proof:}}%
%        {\hspace*{\fill}$\Box$\par}
%\newenvironment{proofof}[1]%{\smallskip\noindent{\bf Proof of #1:}}
%        {\hspace*{\fill}$\Box$\par}

\newtheorem{theorem}{Theorem}
\newtheorem{thm}{Theorem}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{lemma}{Lemma}
\newtheorem{claim}[lemma]{Claim}
\newtheorem{definition}{Definition}

% I "took" all the \commentts so added D:
\newcommand{\dana}[1]{ {\color{magenta} {\textbf [D: {#1}]}}}
\newcommand{\talya}[1]{ {\textbf{\color{red} [T: #1]}}}
\newcommand{\tnew}[1]{{\color{red} #1}}
\newcommand{\tfootnote}[1]{\footnote{\textcolor{red}{#1}}}
\newcommand{\dnew}[1]{{\color{magenta} #1}}
\newcommand{\rnew}[1]{{\color{cyan} #1}}
\newcommand{\rrnew}[1]{{\color{purple} #1}}

\newcommand{\old}[1]{}
\newcommand{\told}[1]{\textcolor{gray}{#1} }

\newcommand{\ronitt}[1]{\textbf{\color{purple} [Ronitt: #1]}}
\newcommand{\reut}[1]{ {\textbf{\color{cyan} [R: #1]}}}
% \newcommand{\tnew}[1]{{\color{red}{#1}}}

\newcommand{\SodaReb}[1]{{\color{blue} #1}}

% \newcommand{\ForFuture}[1]{ {\textbf{\color{red} [ForFuture: #1]}}}
\newcommand{\ForFuture}[1]{}

\makeatletter
\def\moverlay{\mathpalette\mov@rlay}
\def\mov@rlay#1#2{\leavevmode\vtop{%
   \baselineskip\z@skip \lineskiplimit-\maxdimen
   \ialign{\hfil$\m@th#1##$\hfil\cr#2\crcr}}}
\newcommand{\charfusion}[3][\mathord]{
    #1{\ifx#1\mathop\vphantom{#2}\fi
        \mathpalette\mov@rlay{#2\cr#3}
      }
    \ifx#1\mathop\expandafter\displaylimits\fi}
\makeatother

\newcommand{\cupdot}{\charfusion[\mathbin]{\cup}{\cdot}}
\newcommand{\bigcupdott}{\charfusion[\mathop]{\bigcup}{\cdot}}

\newenvironment{packed_enum}{
\begin{enumerate}
  \setlength{\itemsep}{0pt}
  \setlength{\parskip}{0pt}
  \setlength{\parsep}{0pt}
}{\end{enumerate}}

%%%%%%%%%%%%%%%
\iffalse
 \newcommand{\SelectEdge}{\hyperref[alg:select-edge]{\color{black}{\sf Select-an-Edge}}}
  \newcommand{\TestCfour}{\hyperref[alg:C4]{\color{black}{\sf Test-$C_4$-freeness}}}
 \newcommand{\TestCfive}{\hyperref[alg:C5]{\color{black}{\textsf{Test-$C_5$-freeness}}}}
\newcommand{\TestCsix}{\hyperref[alg:C6]{\color{black}{\textsf{Test-$C_6$-freeness}}}}
\newcommand{\TestCk}{\hyperref[alg:Ck]{\color{black}{\textsf{Test-$C_k$-freeness}}}}
\newcommand{\TestFfree}{\hyperref[alg:Ffree]{\color{black}{\textsf{Test-subgraph-freeness}}}}
\fi
%%%%%%%%%%%%%%%%%


\newcommand{\preprocess}{\hyperref[alg:preprocess]{\color{black}{\sf Construct-Data-Structure}}}

 \newcommand{\sampHighVertex}{\hyperref[alg:sampHigh]{\color{black}{\sf Sample-Medium-High-Vertex}}}

\newcommand{\sampLowCycles}{\hyperref[alg:sampLowCycles]{\color{black}{\sf Sample-Low-Cycle}}}

\newcommand{\sampHMCycles}{\hyperref[alg:sampHMCycles]
{\color{black}{\sf Sample-Mixed-Cycle}}}

\newcommand{\sampLowCopies}{\hyperref[alg:sampLowCopies]{\color{black}{\sf Sample-Low-Copy}}}

\newcommand{\sampHMCopies}{\hyperref[alg:sampHMCopies]
{\color{black}{\sf Sample-Mixed-Copy}}}


\newcommand{\sampHighCliques}{\hyperref[alg:sampHighCliques]
{\color{black}{\sf Sample-High-Clique}}}

\newcommand{\sampMediumCliques}{\hyperref[alg:sampMediumClique]
{\color{black}{\sf Sample-Medium-Clique}}}

\newcommand{\sampLowCliques}{\hyperref[alg:sampLowClique]
{\color{black}{\sf Sample-Low-Clique}}}

\newcommand{\sampMHStar}{\hyperref[alg:sampMixed]
{\color{black}{\sf Sample-Not-Low-Star}}}



\newcommand{\ApproxWithEstimate}
{\hyperref[alg:approx-with-estimate]{\color{black}{\sf Approximate-Counting-with-Advice}}}

\newcommand{\SampleWithEstimate}
{\hyperref[alg:sample-copy]{\color{black}{\sf Sample-Copy}}}

\newcommand{\sampleAdvice}
{\hyperref[alg:sample-copy]{\color{black}{\sf Sample-Copy}}}


\newcommand{\SampleCliqueWithEstimate}
{\hyperref[alg:sample-clique]{\color{black}{\sf Sample-Clique}}}

\newcommand{\approxCountWithAdvice}
{\hyperref[alg:approx-count-with-advice]{\color{black}{\sf Approx-Count-with-Advice}}}

\newcommand{\SampleStarsWithAdvice}
{\hyperref[alg:sample-stars-with-advice]{\color{black}{\sf Sample-Star}}}

\newcommand{\Approx}
{\hyperref[alg:approx-search]{\color{black}{\sf Approximate-Counting}}}

\newcommand{\basicSamplerPreprocess}{\hyperref[alg:sampler-preprocess]{\color{black}{\sf Sampler-Preprocessing}}}


 % \textsf{Test-subgraph-freeness}

\newcommand{\sets}{\lceil \frac{n}{\ogamma}\cdot \frac{3\ln(4nt/\delta)}{\oeps^2}\rceil}


 %figure algorithm confFigure
\newcommand{\alg}[1]{\begin{figure*}[htb]
        \centering
		\fbox{
			\begin{minipage}{0.95\textwidth}{
	#1	
}
	\end{minipage}
}
\end{figure*}
}	

\newcommand{\search}{{\sf Search}}
\newcommand{\algA}{\calA}
\newcommand{\ApproxCliquesEstimate}{\textsf{Approx-Count-Cliques-With-Estimate}}
\newcommand{\ok}{\overline{n}_{\textsf{K}}}
\newcommand{\hk}{\hat{n}_{\textsf{K}}}
\newcommand{\invokeA}{\mathcal{A}}
\newcommand{\ov}{\overline{v}}
%\newcommand{\vv}{v}
\newcommand{\vvv}{v}
\newcommand{\hv}{\hat{v}}
\newcommand{\ert}[1]{E_{rt}\left(#1\right)}

\newcommand{\nS}{n_{\textsf{S}}}
 \newcommand{\onS}{\overline{n}_{\textsf{S}}}
 \newcommand{\odmax}{\overline{d}_{max}}

\newcommand{\otheta}{\overline{\theta}}
\newcommand{\samplerAdvice}{\textsf{Sampler-With-Advice}}
\newcommand{\samplerPreprocess}{\textsf{Sampler-Preprocessing}}
\newcommand{\sampler}{\textsf{Sampler}}
\newcommand{\approxCounter}{\sf{Approx-Count}}


==> stars-for-full-version.tex <==


\alg{
	{\bf \sampMHStar}$\;(n,k,\ogamma,\om,\calD,\onS)$ \label{alg:sampMixed}
	\smallskip
	\begin{enumerate}[itemsep=.2em]
 \item Let $\odmax=\min\{q,n\}$, where $q$  is the maximal integer such that $\binom{q}{k-1}\leq 4\onS$.
            \item Invoke \sampHighVertex$(\calD,\ogamma)$. 
              If no vertex is returned, then
              \textbf{return} \emph{fail}. Otherwise, denote the vertex returned  by $v_1$.
              \item If $d(v_1)> \odmax$ then \textbf{return} \emph{fail}.
             \label{step:mixed-stars-samp-high}
            \item Choose an index $j \in [d(v_1)]$ and query for $v_1$'s $j\th$ neighbor. Let this vertex be denoted $v_2$.\label{step:mixed-first-edge} 
              \comment{Sample a uniform neighbor of $v_{1}$.}
             \item \label{mixed-stars:other-edges} For ($y = 3$ to $k$) do: \comment{Sample $k-2$ neighbors of $v_1$, each w.p. $1/\odmax$.}
              \begin{enumerate}
                \item Choose an index $j\in [\odmax]$  u.a.r. 
                If $j>d(v_1)$, then \textbf{return} \emph{fail}. 
                Otherwise query for $v_1$'s $j\th$ neighbor and let $v_y$ denote the neighbor returned.  
              \label{step:hm-sample-neighbor-light}
          \end{enumerate}
      \item \label{step:check-cycle} If 
      for any pair $y\neq y'$, $v_y=v_{y'}$, then \textbf{return} \emph{fail}.
      \comment{Verify that no vertex is sampled twice.}
      \item Verify that $v_2 \prec \ldots \prec v_{k}$. Otherwise, \textbf{return} \emph{fail}.
    \item Return the star  $v_1, \ldots, v_{k}$.
  \end{enumerate}
  }

\begin{lemma}
Consider an invocation of \sampMHStar$(n,s,\ogamma,\om,\calD, \onS)$, and assume that $\calD$ is an $(\oeps,\ogamma,\om)$-degrees typical data structure. 
If $\onS\geq \nS/4$, then every non-low copy of $k$-star in $G$ is returned with probability $\frac{1}{\om\cdot (\min\{q,n\})^{k-2}}$ for $q$ which is the, maximal integer such that $\binom{q}{k-1}\leq 4\onS$.

% If $\onS<\nS$ then only copies incident to vertices with degree at most $q$ may be sampled, and each such copy is sampled with probability $\frac{1}{m\cdot (\min\{(4\onS)^{1/s},n\})^{s-1}}$.

The query complexity and running time of the procedure are $O(k)$.
\end{lemma}
\begin{proof}
Assume that  $\onS\geq \nS/4$, 
and let $q$ denote the maximum value such that $\binom{q}{k-1}\leq 4\onS$ (so that $q=\Theta(\onS^{1/(k-1)})$). 
Then for every $v$, $d(v)\leq q$, as otherwise the number of $k$-stars in the graph will exceed $4\onS$ which in turn exceeds $\nS$. Hence, $\odmax=\min\{q, n\}$ is an upper bound ont the maximum degree in the graph. 
Thus, every non-low copy is sampled with probability in $$(1\pm\oeps)\cdot \frac{d(v)}{2\om}\cdot \frac{1}{d(v)}\cdot \frac{1}{\odmax^{k-2}}=(1\pm\oeps)\cdot \frac{1}{2\om\cdot \odmax^{k-2}}.$$

The query complexity and running time are clear from the description of the algorithm.
\end{proof}

     


\alg{
	{\bf \SampleStarsWithAdvice}$\;(k,\ogamma, \om, \calD, p_1, p_2)$ \label{alg:sample-stars-with-advice}
	\smallskip
	\begin{enumerate}[itemsep=.2em]
 \item Set $\odmax=\min\{q,n\}$, where $q$  is the maximal integer such that $\binom{q}{k-1}\leq 4\onS$.
       \item Set $\Bl =  n\cdot \ogamma^k$,\; $\Bmh =  2\om \cdot \odmax^{k-2}$\;.
       \item \label{step:samp-copy} With probability $\frac{\Bl}{\Bl + \Bmh}$ invoke the above describe sampling procedure for low copies  with parameters $s$ and $\ogamma$, and with probability $\frac{\Bmh}{\Bl + \Bmh}$ invoke \sampMHStar$(n,k,\ogamma,\om,\calD,\onS)$.
       \item If a copy of $\F$ was returned, then return this copy. Otherwise \textbf{return} \emph{fail}. 
       \end{enumerate}
 \vspace{.5em}
}


==> summaries.tex <==
% \documentclass{article}
% \usepackage[utf8]{inputenc}
% \usepackage{hyperref}
% \usepackage{fullpage}
% \usepackage{amsmath}
% \title{subgraph freeness}
% \author{talyaa01}
% \date{February 2022}

% \newcommand{\eps}{\epsilon}
% \newcommand{\light}{\textsf{light}}
% \newcommand{\heavy}{\textsf{heavy}}
% \renewcommand{\ll}{\textsf{$\ell-\ell$}}
% \newcommand{\hh}{\textsf{$h-h$}}
% \newcommand{\lh}{\textsf{$\ell-h$}}
% \newcommand{\davg}{d_{avg}}
% \newcommand{\poly}{\textrm{poly}}

% \begin{document}

\section{Meeting 30/1/2024}
Hi,

 

We have photographs of the board, but I thought it won’t hurt to have it also in text.

[To Reut: we didn’t do much more after you left, just very quick verified a couple of things.]

 

In terms of the tasks we wrote for ourselves on the board.

 

1. Even-length cycles:

    - Upper bound of $O(n/(#C_k)^{1/k} + m^{k/2}/#C_k)$. We thought we had it for $k=4$, and believe it was true for any even $k$, but then had trouble with the variance analysis. So we took another direction, that seems to work for $k=4$ and hopefully extends beyond. A bit more on this below.

    - Lower bound. Most probably not matching (for the second term – the first term is trivial, based on hitting a clique of size $(#C_k)^{{1/k}$). Did not talk about this.

    - Handling the gap we believe there is between the upper and lower bound (the upper bound may be lower).

 

2. Odd-Length cycles.

   - Here there is a lower bound of $\Omega(n/(#C_k)^{1/k} + m^{k/2}/#C_k))|$. Again, the first term is just a trivial, and we talked about the second. Roughly based on a blow-up of a path of length $k$ between sets of size $\sqrt{m}$ (or smaller for smaller #C_k) with complete bipartite graphs between them.

  - Didn’t talk about the upper bound, but hopefully, if things work out for even-length cycles with the current approach, then it extends to odd length cycles.

 

3. General $H$.

 

I think the best thing next time is to first verify that the current approach indeed generalizes to any even-length cycle, then continue to odd-length cycles, and if all this works nicely… attack general $H$.

 

Regarding the current approach, will write below the structure for $C_4$.

 

In terms of the algorithm, it is similar to the previous one, but the assignment rule is different, which affects the analysis as well as the algorithm itself in its last step. In what follows I am ignoring the dependence on $\epsilon$, and will use $C$ instead of $#C_k$ (in any case, we’ll probably need to select a different notation). We are also assuming here that we have a constant factor estimate of $C$ (which is used for setting the sample sizes).

 

1. Select two (multi)sets, $R_1$, and $R_2$, each of size $r = O(n/C^{1/4})$ (iid vertices).

 

2. Query all degrees of vertices in the two sets. The sums of the degrees of vertices in $R_b$ is $m_{R_b}$, and we denote the set of edges itself by $E_{R_b}$.

 

3. Repeat the following $s = O(m^2/C)$ times: select a random edge $(u_1,v_1)$ from $E_{R_1}$ and a random edge $(u_2,v_2)$ from $E_{R_2}$. Query to see if we get a $4$-cycles on these four vertices.

 

4. For each $4$-cycle we got, check whether it is assigned to $u_1$ as a “primary leader” (different term?) and to $u_2$ as a “secondary leader”.

 

5. Output the estimate based on the number of $4$-cycles that were assigned as required above (using an appropriate normalizing).

 

We need to explain and show:

 

1.  What is the assignment rule, and why is it the case that at most $\epsilon C$ cycles remain unassigned (because they don’t have a primary leader or a secondary leader). This involves setting cycle-heaviness thresholds and degree-highness thresholds.

 

2.  Why does the setting of $r$ ensure that whp over the choice of $R_1$, the number of cycles assigned to $R_1$, i.e., whose primary leader is in $R_1$, is close to its expected value (which is $r C / n$). We denote the number of these assigned cycles by $as(R_1)$, and their set by $AS(R_1).

 

3. Why does the setting of $r$ ensure that whp, among the cycles in $AS(R_1)$, the number of them assigned to $R_2$ (in a secondary manner, i.e., whose secondary leader is in $R_2$), is close to its expected value (which is $r ass(R_1) / n$). We denote the number of these cycles by $as(R_1,R_2)$, and their set by $AS(R_1,R_2)$.

 

4. Why does the setting of $s$ ensure that whp the number of $4$-cycles that we get is close to its expected value (which is $as(R_1,R_2)/(m_{R_1} m_{R_2})$). Also need to verify that this expected value is a constant or maybe polylogish.

 

5. How do we check that a cycle on  $\{u_1,v_1,u_2,v_2\}$ is assigned to $u_1$ (primary) and $u_2$ (secondary), and what is the complexity of this check per cycle?

 

I can start writing some answers to the above, but this email is starting to get a bit long, so maybe we’ll go over these questions when we check general even-length cycles (where the algorithm is generalized to selecting $R_1,…,R_{k/2}$, repeatedly selecting an edge from each, checking that these edges are part of a cycle, and then checking the cycle is assigned as required).


% \end{document}

